HeLiMOS: A Dataset for Moving Object Segmentation in 3D Point Clouds From Heterogeneous LiDAR Sensors

Moving object segmentation (MOS) using a 3D light detection and ranging (LiDAR) sensor is crucial for scene understanding and identification of moving objects. Despite the availability of various types of 3D LiDAR sensors in the market, MOS research still predominantly focuses on 3D point clouds from mechanically spinning omnidirectional LiDAR sensors. Thus, we are, for example, lacking a dataset with MOS labels for point clouds from solid-state LiDAR sensors which have irregular scanning patterns. In this paper, we present a labeled dataset, called \textit{HeLiMOS}, that enables to test MOS approaches on four heterogeneous LiDAR sensors, including two solid-state LiDAR sensors. Furthermore, we introduce a novel automatic labeling method to substantially reduce the labeling effort required from human annotators. To this end, our framework exploits an instance-aware static map building approach and tracking-based false label filtering. Finally, we provide experimental results regarding the performance of commonly used state-of-the-art MOS approaches on HeLiMOS that suggest a new direction for a sensor-agnostic MOS, which generally works regardless of the type of LiDAR sensors used to capture 3D point clouds. Our dataset is available at https://sites.google.com/view/helimos.

==> figures/data_statistics.tex <==
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{pics/fig6/fig6_cluster_1.png}
        \includegraphics[width=1.0\textwidth]{pics/fig6/C1_bold.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{pics/fig6/fig6_cluster_2.png}
        \includegraphics[width=1.0\textwidth]{pics/fig6/C2_bold.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{pics/fig6/fig6_cluster_3.png}
        \includegraphics[width=1.0\textwidth]{pics/fig6/C3_bold.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.22\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{pics/fig6/fig6_cluster_4.png}
        \includegraphics[width=1.0\textwidth]{pics/fig6/C4_bold.pdf}
    \end{subfigure}
    \captionsetup{font=footnotesize}
    \caption{(T-B, L-R):~Dynamic points ratios, each of which is defined as $\frac{\text{\# of labeled dynamic points}}{\text{\# of total points in the $t$-th scan}}$, over time steps and the visualized cleaned point cloud maps of four subclusters, corresponding to $\mathcal{C}_1$, $\mathcal{C}_2$, $\mathcal{C}_3$, and $\mathcal{C}_4$ in \figref{fig:clustering}(d).
    \changed{Note that} the MOS labels of our HeLiMOS show a variety of dynamic point patterns owing to the varying trajectories of moving objects even though the scans are acquired in the same places.
    \changed{This is because the point clouds in our dataset are from the HeLiPR dataset which is originally designed for place recognition tasks to evaluate whether a robot revisits the same location; thus, our dataset also includes scans captured at the same locations multiple times at different moments.}
    Red points indicate the annotated points, which are traces of moving objects~(best viewed in color).}
    \label{fig:data_statistics}
    \vsfig
\end{figure*}


==> figures/heli_kitti_poss.tex <==
\begin{figure}[t]
  \centering
  \begin{subfigure}[b]{0.44\textwidth}
    \centering
    \includegraphics[width=1.0\textwidth]{pics/fig6/comparison_w_kiiti_poss2.png}
    \end{subfigure}
    \captionsetup{font=footnotesize}
    \caption{Comparison of dynamic points ratio with other datasets. The numbers on the bars represent the average ratios, while the black error bars indicate the standard deviations.
    For calculating the dynamic points ratio of SemanticKITTI~\cite{behley2019iccv}, we counted the points labeled as moving objects.
    As described in \tabref{table:summary}, the SemanticPOSS~\cite{pan2020semanticposs} wrongly classifies parked vehicles as moving objects.
    Thus, for a fair comparison, we filtered out them using our tracking-based filtering and only used the actual moving objects for the dynamic points ratio calculation.}
  \label{fig:heli_kitti_poss}
  \vsfig
\end{figure}


==> figures/heli_lidar_viz.tex <==
\begin{figure}[t]
    \captionsetup{font=footnotesize}
    \centering
    \begin{subfigure}[b]{0.11\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{pics/fig7/bicycle_a.png}
        \includegraphics[width=1.0\textwidth]{pics/fig7/bicycle_l.png}
        \includegraphics[width=1.0\textwidth]{pics/fig7/bicycle_o.png}
        \includegraphics[width=1.0\textwidth]{pics/fig7/bicycle_v.png}
        \caption{}
    \end{subfigure}
    \begin{subfigure}[b]{0.11\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{pics/fig7/person_a.png}
        \includegraphics[width=1.0\textwidth]{pics/fig7/person_l.png}
        \includegraphics[width=1.0\textwidth]{pics/fig7/person_o.png}
        \includegraphics[width=1.0\textwidth]{pics/fig7/person_v.png}
        \caption{}
    \end{subfigure}
    \begin{subfigure}[b]{0.11\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{pics/fig7/car_a.png}
        \includegraphics[width=1.0\textwidth]{pics/fig7/car_l.png}
        \includegraphics[width=1.0\textwidth]{pics/fig7/car_o.png}
        \includegraphics[width=1.0\textwidth]{pics/fig7/car_v.png}
        \caption{}
    \end{subfigure}
     \begin{subfigure}[b]{0.11\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{pics/fig7/truck_a.png}
        \includegraphics[width=1.0\textwidth]{pics/fig7/truck_l.png}
        \includegraphics[width=1.0\textwidth]{pics/fig7/truck_o.png}
        \includegraphics[width=1.0\textwidth]{pics/fig7/truck_v.png}
        \caption{}
    \end{subfigure}
    \vsfigu
    \caption{Examples of moving objects in our dataset, which are shown as red points. From top to bottom, these examples show the zoomed point clouds captured by Aeva Aeries~\rom{2}, Livox Avia, Ouster OS2-128, and Velodyne VLP-16. Note that even though the same objects are shown, they have different patterns owing to the difference in scanning techniques and field of views of the sensors. MOS labels of (a)~a bicyclist and pedestrian, (b)~crowded pedestrians, (c)~a car, and (d)~a truck~(best viewed in color).}
    \label{fig:heli_lidar_viz}
    \vsfig
\end{figure}


==> figures/sota_static_map_building_comparison.tex <==
\begin{figure}[t]
    \captionsetup{font=footnotesize}
    \centering
    \begin{subfigure}[b]{0.13\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{pics/fig10/2250_2500_rmv.png}
        \includegraphics[width=1.0\textwidth]{pics/fig10/8600_8800_rmv.png}
        \includegraphics[width=1.0\textwidth]{pics/fig10/11070_11300_rmv.png}
        \caption{Removert~\cite{kim2020iros}}
    \end{subfigure}
    \begin{subfigure}[b]{0.13\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{pics/fig10/2250_2500_ers1.png}
        \includegraphics[width=1.0\textwidth]{pics/fig10/8600_8800_ers1.png}
        \includegraphics[width=1.0\textwidth]{pics/fig10/11070_11300_ers1.png}
        \caption{ERASOR~\cite{lim2021ral}}
    \end{subfigure}
    \begin{subfigure}[b]{0.13\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{pics/fig10/2250_2500_ers2.png}
        \includegraphics[width=1.0\textwidth]{pics/fig10/8600_8800_ers2.png}
        \includegraphics[width=1.0\textwidth]{pics/fig10/11070_11300_ers2.png}
        \caption{ERASOR2~\cite{lim2023erasor2}}
    \end{subfigure}
    \vsfigu
    \caption{(a)-(c) Qualitative comparison of static map building results produced by state-of-the-art methods on our dataset using synced scans.
    Green, red, and blue points indicate true positives, false positives, and false negatives, respectively. The fewer red and blue points there are, the better~(best viewed in color).}
    \label{fig:sota_static_map_building_comparison}
    \vsfig
\end{figure}


==> tables/comparison_of_tracking.tex <==
\begin{table}[t!]
	\centering
	\captionsetup{font=footnotesize}
	\caption{Mean IoU before and after the application of tracking-based filtering approaches.}
%	\setlength{\tabcolsep}{5pt}
	{\scriptsize
	\begin{tabular}{lcccc}
		\toprule \midrule
		Method & $\iou$ \\ \midrule
		% \multirow{3}{*}{\begin{tabular}{@{}c@{}}2,250- \\ 2,500 \end{tabular}}
		ERASOR2~\cite{lim2023erasor2}   &  21.4 \\
		ERASOR2 + Tracking-based filtering in Auto-MOS~\cite{chen2022ral} & 25.2     \\
		ERASOR2 + Our tracking-based filtering & \textbf{34.8} \\ \midrule
		\bottomrule
	\end{tabular}
	}
	\label{table:comparison_of_tracking}
\end{table}


==> tables/comparison_of_tracking_0724.tex <==
\begin{table}[t!]
	\centering
	\captionsetup{font=footnotesize}
	\caption{Mean IoU before and after the application of tracking-based filtering approaches.}
%	\setlength{\tabcolsep}{5pt}
	{\scriptsize
	\begin{tabular}{lcccc}
		\toprule \midrule
		Method & $\iou$ \\ \midrule
		% \multirow{3}{*}{\begin{tabular}{@{}c@{}}2,250- \\ 2,500 \end{tabular}}
		ERASOR2~\cite{lim2023erasor2}   &  21.8 \\
		ERASOR2 + Tracking-based filtering in Auto-MOS~\cite{chen2022ral} & 53.4     \\
		ERASOR2 + Our tracking-based filtering & \textbf{61.2} \\ \midrule
		\bottomrule
	\end{tabular}
	}
	\label{table:comparison_of_tracking}
\end{table}


==> tables/cross_sensor_config.tex <==
\begin{table}[t!]
	\centering
	\captionsetup{font=footnotesize}
	\caption{Mean IoU of MOS approaches when trained solely on data from specific LiDAR sensors.
	The bold and the gray highlight indicate the best performance among all trials and that for each training dataset within each test set, respectively~($\texttt{L}$:~Livox Avia, $\texttt{A}$:~Aeva Aeries~\rom{2}, $\texttt{O}$:~Ouster OS2-128, and $\texttt{V}$:~Velodyne VLP-16).}
	\setlength{\tabcolsep}{3.5pt}
	{\scriptsize
		\begin{tabular}{clccccccc}
			\toprule \midrule
			\multirow{2}{*}[-0.5em]{Train data} & \multirow{2}{*}[-0.5em]{Method}  & \multicolumn{3}{c}{Solid-state} & \multicolumn{3}{c}{Omnidirectional}          & \multirow{2}{*}[-0.5em]{Total}    \\ \cmidrule(lr){3-5} \cmidrule(lr){6-8}
			                                    &                                  & \texttt{L}                      & \texttt{A}                          & Avg   & \texttt{O} & \texttt{V} & Avg &    \\ \midrule
			%%%%%%%%% 00 %%%%%%%%%%
			\multirow{2}{*}[-0.0em]{\texttt{L}+\texttt{A}} & 4DMOS~\cite{mersch2022ral}       & 65.76                      & 77.62                & 71.69 & 70.04      & \hl{35.86}      & 52.95 & 62.32\\
			                                    & MapMOS~\cite{mersch2023building} & \hl{\textbf{72.84}}        & \hl{80.24}           & \hl{\textbf{76.54}} & \hl{\textbf{80.23}}      & 33.98      & \hl{57.11} & \hl{66.82} \\ \midrule
			\multirow{2}{*}[-0.0em]{\texttt{O}+\texttt{V}}  & 4DMOS~\cite{mersch2022ral}       & 50.26                      & 65.08                & 57.67 & 73.88      & \hl{\textbf{55.39}}      & 64.64 & 61.15 \\
			                                    & MapMOS~\cite{mersch2023building} & \hl{56.80}                 & \hl{78.29}           & \hl{67.56} & \hl{78.85}      & 50.72      & \hl{\textbf{64.79}} & \hl{66.17} \\ \midrule
			\multirow{2}{*}[-0.0em]{All}        & 4DMOS~\cite{mersch2022ral}       & 63.53                      & 75.26                & 69.40 & 74.36      & \hl{49.95}      & \hl{62.16} & 65.78 \\
			                                    & MapMOS~\cite{mersch2023building} & \hl{72.03}                 & \hl{\textbf{80.30}}  & \hl{76.17} & \hl{78.08}      & 41.95      & 60.02 & \hl{\textbf{68.09}} \\
			\midrule \bottomrule
		\end{tabular}
	}
	\label{table:cross_sensor_config}
\end{table}


==> tables/cross_sensor_config_0307.tex <==
\begin{table}[t!]
	\centering
	\captionsetup{font=footnotesize}
	\caption{Mean IoU of MOS approaches when trained solely on data from specific LiDAR sensors.
		The bold and the gray highlight indicate the best performance among all trials and that for each training dataset within each test set, respectively~($\texttt{L}$:~Livox Avia, $\texttt{A}$:~Aeva Aeries~\rom{2}, $\texttt{O}$:~Ouster OS2-128, and $\texttt{V}$:~Velodyne VLP-16).}
	\setlength{\tabcolsep}{3.5pt}
	{\scriptsize
		\begin{tabular}{clccccccc}
			\toprule \midrule
			\multirow{2}{*}[-0.5em]{Train data}            & \multirow{2}{*}[-0.5em]{Method}  & \multicolumn{3}{c}{Solid-state} & \multicolumn{3}{c}{Omnidirectional} & \multirow{2}{*}[-0.5em]{Total}                                                                                         \\ \cmidrule(lr){3-5} \cmidrule(lr){6-8}
			                                               &                                  & \texttt{L}                      & \texttt{A}                          & Avg                            & \texttt{O}          & \texttt{V}          & Avg                 &                     \\ \midrule
			%%%%%%%%% 00 %%%%%%%%%%
			\multirow{2}{*}[-0.0em]{\texttt{L}+\texttt{A}} & 4DMOS~\cite{mersch2022ral}       & 63.44                           & 80.09                               & 71.77                          & 73.29               & \hl{51.28}          & \hl{62.29}          & 67.01               \\
			                                               & MapMOS~\cite{mersch2023building} & \hl{\textbf{72.86}}             & \hl{81.38}                          & \hl{\textbf{77.12}}            & \hl{81.46}          & 38.13               & 59.80               & \hl{68.46}          \\ \midrule
			\multirow{2}{*}[-0.0em]{\texttt{O}+\texttt{V}} & 4DMOS~\cite{mersch2022ral}       & 44.78                           & 66.00                               & 55.39                          & 77.02               & \hl{54.44}          & 65.73               & 60.56               \\
			                                               & MapMOS~\cite{mersch2023building} & \hl{62.61}                      & \hl{77.21}                          & \hl{69.91}                     & \hl{79.38}          & 52.85               & \hl{66.12}          & \hl{68.01}          \\ \midrule
			\multirow{2}{*}[-0.0em]{All}                   & 4DMOS~\cite{mersch2022ral}       & 68.13                           & \hl{\textbf{81.85}}                 & 74.99                          & 78.71               & \hl{\textbf{57.57}} & \hl{\textbf{68.14}} & \hl{\textbf{71.57}} \\
			                                               & MapMOS~\cite{mersch2023building} & \hl{72.55}                      & 80.18                               & \hl{76.37}                     & \hl{\textbf{83.53}} & 43.74               & 63.64               & 70.00               \\
			\midrule \bottomrule
		\end{tabular}
	}
	\label{table:cross_sensor_config}
\end{table}


==> tables/cross_sensor_config_0307_v2.tex <==
\begin{table}[t!]
	\centering
	\captionsetup{font=footnotesize}
	\caption{Mean IoU of MOS approaches when trained solely on data from specific LiDAR sensors.
		The bold texts denote the best performance among all trials and the gray highlights indicate the best results for each method across different training data scenarios~($\texttt{L}$:~Livox Avia, $\texttt{A}$:~Aeva Aeries~\rom{2}, $\texttt{O}$:~Ouster OS2-128, and $\texttt{V}$:~Velodyne VLP-16).}
	\setlength{\tabcolsep}{3.5pt}
	{\scriptsize
		\begin{tabular}{lcccccccc}
			\toprule \midrule
			 \multirow{2}{*}[-0.5em]{Method} & \multirow{2}{*}[-0.5em]{Training data}             & \multicolumn{3}{c}{Solid-state} & \multicolumn{3}{c}{Omnidirectional} & \multirow{2}{*}[-0.5em]{Total}                                                                                         \\ \cmidrule(lr){3-5} \cmidrule(lr){6-8}
			                                               &                                  & \texttt{L}                      & \texttt{A}                          & Avg                            & \texttt{O}          & \texttt{V}          & Avg                 &                     \\ \midrule
			%%%%%%%%% 00 %%%%%%%%%%
			\multirow{3}{*}[-0.0em]{4DMOS~\cite{mersch2022ral}} & {\texttt{L}+\texttt{A}} & 63.44                      & 80.09                     & 71.77                     & 73.29               & 51.28          & 62.29          & 67.01               \\
			                                                    & {\texttt{O}+\texttt{V}} & 44.78                      & 66.00                     & 55.39                     & 77.02               & 54.44          & 65.73               & 60.56               \\
			                                                    & {All}                   & \hl{68.13}                 & \hl{\textbf{81.85}}       & \hl{74.99}                & \hl{78.71}               & \hl{\textbf{57.57}} & \hl{\textbf{68.14}} & \hl{\textbf{71.57}} \\ \midrule
			\multirow{3}{*}[-0.0em]{MapMOS~\cite{mersch2023building}} & {\texttt{L}+\texttt{A}}  & \hl{\textbf{72.86}}        & \hl{81.38}                & \hl{\textbf{77.12}}       & 81.46          & 38.13               & 59.80               & 68.46          \\
			& {\texttt{O}+\texttt{V}} & 62.61                      & 77.21                     & 69.91                     & 79.38          & \hl{52.85}               & \hl{66.12}          & 68.01          \\
			& {All}                   & 72.55                      & 80.18                     & 76.37                     & \hl{\textbf{83.53}} & 43.74               & 63.64               & \hl{70.00}               \\
			\midrule \bottomrule
		\end{tabular}
	}
	\label{table:cross_sensor_config}
\end{table}


==> tables/cross_sensor_config_0724.tex <==
\begin{table}[t!]
	\centering
	\captionsetup{font=footnotesize}
	\caption{Mean IoU of MOS approaches when trained solely on data from specific LiDAR sensors.
		The bold texts denote the best performance among all trials and the gray highlights indicate the best results for each method across different training data scenarios~($\texttt{L}$:~Livox Avia, $\texttt{A}$:~Aeva Aeries~\rom{2}, $\texttt{O}$:~Ouster OS2-128, and $\texttt{V}$:~Velodyne VLP-16).}
	\setlength{\tabcolsep}{3.5pt}
	{\scriptsize
		\begin{tabular}{lcccccccc}
			\toprule \midrule
			 \multirow{2}{*}[-0.5em]{Method} & \multirow{2}{*}[-0.5em]{Training data}             & \multicolumn{3}{c}{Solid-state} & \multicolumn{3}{c}{Omnidirectional} & \multirow{2}{*}[-0.5em]{Total}                                                                                         \\ \cmidrule(lr){3-5} \cmidrule(lr){6-8}
			                                               &                                  & \texttt{L}                      & \texttt{A}                          & Avg                            & \texttt{O}          & \texttt{V}          & Avg                 &                     \\ \midrule
			%%%%%%%%% 00 %%%%%%%%%%
			\multirow{3}{*}[-0.0em]{4DMOS~\cite{mersch2022ral}} & {\texttt{L}+\texttt{A}} & 72.82                      & 81.58                     & 77.20                     & 72.46               & 47.65          & 70.34          & 68.63               \\
			                                                    & {\texttt{O}+\texttt{V}} & 65.13                      & 74.96                     & 70.05                     & 80.50               & 56.09          & 69.35               & 69.17               \\
			                                                    & {All}                   & \hl{73.72}                 & \hl{84.80}       & \hl{79.26}                & \hl{82.70}               & \hl{\textbf{57.64}} & \hl{\textbf{75.63}} & \hl{\textbf{74.72}} \\ \midrule
			\multirow{3}{*}[-0.0em]{MapMOS~\cite{mersch2023building}} & {\texttt{L}+\texttt{A}}  & \hl{\textbf{75.46}}        & {83.65}                & 79.55       & 77.84          & 25.62               & 68.42               & 65.64          \\
			& {\texttt{O}+\texttt{V}} & 75.00                      & 80.71                     & 77.85                     & \hl{\textbf{87.56}}          & \hl{49.13}               & \hl{74.05}          & \hl{73.10}          \\
			& {All}                   & 75.38                      & \hl{\textbf{85.60}}                     & \hl{\textbf{80.49}}                     & {87.31} & 32.00               & 72.15               & 70.07               \\
			\midrule \bottomrule
		\end{tabular}
	}
	\label{table:cross_sensor_config}
\end{table}


==> tables/kitti2helimos.tex <==

\begin{table}[t!]
	\centering
	\captionsetup{font=footnotesize}
	\caption{Mean IoU of MOS approaches trained on the SemanticKITTI dataset to evaluate generalization capabilies in terms of both environmental changes and LiDAR sensor variations. The symbol \xmarkblack$\,$ indicates the approaches are not directly available because those are range image-based approaches ($\texttt{L}$:~Livox Avia, $\texttt{A}$:~Aeva Aeries~\rom{2}, $\texttt{O}$:~Ouster OS2-128, and $\texttt{V}$:~Velodyne VLP-16).}
	{\scriptsize
	\begin{tabular}{lccccc}
		\toprule \midrule
		\multirow{2}{*}[-0.2em]{Method} & \multicolumn{2}{c}{Solid-state} & \multicolumn{2}{c}{Omnidirectional} & \multirow{2}{*}[-0.2em]{Total}  \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5}
		  & \texttt{L} &  \texttt{A} & \texttt{O} & \texttt{V} \\ \midrule
		%%%%%%%%% 00 %%%%%%%%%%
	     LMNet~\cite{chen2021ral} & \xmarkblack & \xmarkblack & \xmarkblack & \xmarkblack & \xmarkblack \\
		 MotionSeg3D~\cite{sun2022mos3d} &  \xmarkblack & \xmarkblack & \xmarkblack & \xmarkblack  & \xmarkblack \\
		 RVMOS~\cite{kim2022ral-rvmos} &  \xmarkblack & \xmarkblack & \xmarkblack & \xmarkblack  & \xmarkblack \\
		 4DMOS, online~\cite{mersch2022ral} & 46.70 & 63.22 & 66.15 & 21.52 & 49.40  \\
	  	 4DMOS, delayed~\cite{mersch2022ral} & \textbf{52.94} & 69.58 & 72.56 & \textbf{31.63} & \textbf{56.68} \\
		 MapMOS, Scan~\cite{mersch2023building} & 47.80 & 70.56 & 80.74 & 7.05 & 51.54 \\
		 MapMOS, Volume~\cite{mersch2023building} & 50.66 & \textbf{71.85} & \textbf{81.99} & 9.24 & 53.44 \\
		\midrule \bottomrule
	\end{tabular}
	}
	\label{table:kitti2helimos}
\end{table}



==> tables/kitti2helimos_0307.tex <==
% Then as far as I understand, the reason for MOS performance degradation in Velodyne compared with the previous results is that we set the max range as the same as other sensors. So if we set the max range of Velodyne to 50 m, its performance would be better like the previous results;
% do I follow you? Before the exp. part manuscript, I just wanna double check whether I understand it correctly.
\begin{table}[t!]
	\centering
	\captionsetup{font=footnotesize}
	\caption{Mean IoU of MOS approaches trained on the SemanticKITTI dataset to evaluate generalization capabilities in terms of both environmental changes and LiDAR sensor variations ($\texttt{L}$:~Livox Avia, $\texttt{A}$:~Aeva Aeries~\rom{2}, $\texttt{O}$:~Ouster OS2-128, and $\texttt{V}$:~Velodyne VLP-16).}
	{\scriptsize
	\begin{tabular}{lccccc}
		\toprule \midrule
		\multirow{2}{*}[-0.2em]{Method} & \multicolumn{2}{c}{Solid-state} & \multicolumn{2}{c}{Omnidirectional} & \multirow{2}{*}[-0.2em]{Total}  \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5}
		  & \texttt{L} &  \texttt{A} & \texttt{O} & \texttt{V} \\ \midrule
		%%%%%%%%% 00 %%%%%%%%%%
%	     LMNet~\cite{chen2021ral} & \xmarkblack & \xmarkblack & \xmarkblack & \xmarkblack & \xmarkblack \\
%		 MotionSeg3D~\cite{sun2022mos3d} &  \xmarkblack & \xmarkblack & \xmarkblack & \xmarkblack  & \xmarkblack \\
%		 RVMOS~\cite{kim2022ral-rvmos} &  \xmarkblack & \xmarkblack & \xmarkblack & \xmarkblack  & \xmarkblack \\
		 4DMOS, online~\cite{mersch2022ral} & 41.96 & 62.83 & 65.06 & 4.84 & 43.67  \\
	  	 4DMOS, delayed~\cite{mersch2022ral} & \textbf{48.44} & 68.60 & 71.53 & 5.46 & 48.51 \\
		 MapMOS, Scan~\cite{mersch2023building} & 37.60 & 68.28 & 81.24 & 6.86 & 48.50 \\
	 MapMOS, Volume~\cite{mersch2023building} & 45.17 & \textbf{69.32} & \textbf{81.53} & \textbf{9.74} & \textbf{51.44} \\
		\midrule \bottomrule
	\end{tabular}
	}
	\label{table:kitti2helimos}
\end{table}



==> tables/kitti2helimos_0724.tex <==
% Then as far as I understand, the reason for MOS performance degradation in Velodyne compared with the previous results is that we set the max range as the same as other sensors. So if we set the max range of Velodyne to 50 m, its performance would be better like the previous results;
% do I follow you? Before the exp. part manuscript, I just wanna double check whether I understand it correctly.
\begin{table}[t!]
	\centering
	\captionsetup{font=footnotesize}
	\caption{Mean IoU of MOS approaches trained on the SemanticKITTI dataset to evaluate generalization capabilities in terms of both environmental changes and LiDAR sensor variations ($\texttt{L}$:~Livox Avia, $\texttt{A}$:~Aeva Aeries~\rom{2}, $\texttt{O}$:~Ouster OS2-128, and $\texttt{V}$:~Velodyne VLP-16).}
	{\scriptsize
	\begin{tabular}{lccccc}
		\toprule \midrule
		\multirow{2}{*}[-0.2em]{Method} & \multicolumn{2}{c}{Solid-state} & \multicolumn{2}{c}{Omnidirectional} & \multirow{2}{*}[-0.2em]{Total}  \\ \cmidrule(lr){2-3} \cmidrule(lr){4-5}
		  & \texttt{L} &  \texttt{A} & \texttt{O} & \texttt{V} \\ \midrule
		%%%%%%%%% 00 %%%%%%%%%%
%	     LMNet~\cite{chen2021ral} & \xmarkblack & \xmarkblack & \xmarkblack & \xmarkblack & \xmarkblack \\
%		 MotionSeg3D~\cite{sun2022mos3d} &  \xmarkblack & \xmarkblack & \xmarkblack & \xmarkblack  & \xmarkblack \\
%		 RVMOS~\cite{kim2022ral-rvmos} &  \xmarkblack & \xmarkblack & \xmarkblack & \xmarkblack  & \xmarkblack \\
		 4DMOS, online~\cite{mersch2022ral} & 52.08 & 54.01 & 64.17 & 4.69 & 43.74  \\
	  	 4DMOS, delayed~\cite{mersch2022ral} & 58.99 & 58.30 & 70.44 & 5.41 & 48.28 \\
		 MapMOS, Scan~\cite{mersch2023building} & 58.93 & 63.15 & 81.43 & 4.33 & 51.96 \\
	 MapMOS, Volume~\cite{mersch2023building} & \textbf{62.70} & \textbf{66.58} & \textbf{82.87} & \textbf{5.77} & \textbf{54.48} \\
		\midrule \bottomrule
	\end{tabular}
	}
	\label{table:kitti2helimos}
\end{table}



==> tables/static_map_building_in_hetero_lidar.tex <==
\newcommand{\threemetrics}{\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} $\PRmap$ [\%] \end{tabular}}  & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} $\RRmap$ [\%] \end{tabular}} & $\mathrm{F}_{1}$ score}

\begin{table*}[t!]
	\centering
	\captionsetup{font=footnotesize}
	\caption{Comparison with state-of-the-art methods on the static map benchmark using our dataset~($\PRmap$: Preservation Rate, $\RRmap$: Rejection Rate).}
	\setlength{\tabcolsep}{5pt}
	{\scriptsize
	\begin{tabular}{llccccccccccccccc}
		\toprule \midrule
		\multirow{2}{*}[-0.5em]{Seq.} & \multirow{2}{*}[-0.5em]{Method} & \multicolumn{3}{c}{\texttt{L}} & \multicolumn{3}{c}{\texttt{A}} & \multicolumn{3}{c}{\texttt{O}} & \multicolumn{3}{c}{\texttt{V}}  \\ \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14}
			& & \threemetrics & \threemetrics & \threemetrics & \threemetrics \\ \midrule
		\multirow{3}{*}{$\mathcal{C}_1$}
		& Removert~\cite{kim2020iros} & 75.182  & 52.802 & 0.620 & 66.285 & 80.679 & 0.728  & 82.823  & 83.817 & 0.833  & 74.450  & 60.780 & 0.669     \\
		& ERASOR~\cite{lim2021ral} & 83.025	& 85.409 &	0.842 &	92.749 & 73.773 &	0.822 &	87.251 & 96.248 &	0.915 &	87.366 &	67.637 &	0.762   \\
		& ERASOR2~\cite{lim2023erasor2} & 98.788 &  98.582 & 0.987 & 98.788 &  98.582 & 0.987 & 98.788 &  98.582 & 0.987 & 98.788 &  98.582 & 0.987 \\ \midrule
		\multirow{3}{*}{$\mathcal{C}_2$}
		& Removert~\cite{kim2020iros} & 78.886	&50.119	&0.613&	70.683&	68.599	&0.696&	84.820&	77.379	&0.809&	72.704&	57.204	&0.640     \\
		& ERASOR~\cite{lim2021ral} & 89.580 &	73.606 &	0.808	&92.087	&68.993&	0.789&	88.767	&90.654&	0.897	&86.274&	74.076&	0.797   \\
		& ERASOR2~\cite{lim2023erasor2} & 98.788 &  98.582 & 0.987 & 98.788 &  98.582 & 0.987 & 98.788 &  98.582 & 0.987 & 98.788 &  98.582 & 0.987 \\ \midrule
		\multirow{3}{*}{$\mathcal{C}_3$}
		& Removert~\cite{kim2020iros} & 80.454	& 64.626	&0.717&	74.683	&79.541	&0.770&	84.339	&82.039	&0.832&	74.193	&50.525&	0.601     \\
		& ERASOR~\cite{lim2021ral} & 89.271 &	88.538 &	0.889 &	92.431 &	89.455 &	0.909 &	87.357 & 91.800 &	0.895 &	89.567 & 70.272 &	0.788   \\
		& ERASOR2~\cite{lim2023erasor2} & 98.788 &  98.582 & 0.987 & 98.788 &  98.582 & 0.987 & 98.788 &  98.582 & 0.987 & 98.788 &  98.582 & 0.987 \\ \midrule
		\multirow{3}{*}{$\mathcal{C}_4$}
		& Removert~\cite{kim2020iros} & 76.562 &	81.815	&0.791	&70.186&	94.292	&0.805&	81.850	&99.918&	0.900&	74.746	&90.362	& 0.818    \\
		& ERASOR~\cite{lim2021ral} & 78.427	 &97.765 &	0.870&	88.430	&96.482&	0.923	&77.694	&99.277	&0.872	& 80.229&	94.021&	0.866  \\
		& ERASOR2~\cite{lim2023erasor2} & 98.788 &  98.582 & 0.987 & 98.788 &  98.582 & 0.987 & 98.788 &  98.582 & 0.987 & 98.788 &  98.582 & 0.987 \\ \midrule
		\bottomrule
	\end{tabular}
	}
	\label{table:semantic_kitti}
\end{table*}


==> tables/static_map_building_in_synced_scans.tex <==
\newcommand{\threemetrics}{\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} $\PRmap$ [\%] \end{tabular}}  & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} $\RRmap$ [\%] \end{tabular}} & $\text{F}_{1}$ score}

\begin{table}[t!]
	\centering
	\captionsetup{font=footnotesize}
	\caption{Comparison of static map building approaches for the most crowded frame sequences in our dataset~($\PRmap$: Preservation Rate, $\RRmap$: Rejection Rate).}
%	\setlength{\tabcolsep}{5pt}
	{\scriptsize
	\begin{tabular}{clccc}
		\toprule \midrule
		Frame range & Method & \threemetrics \\ \midrule
		\multirow{3}{*}{2,250-2,500}
		% \multirow{3}{*}{\begin{tabular}{@{}c@{}}2,250- \\ 2,500 \end{tabular}}
		& Removert~\cite{kim2020iros}   & 84.615 & 54.836 & 0.665    \\
		& ERASOR~\cite{lim2021ral}      & 95.448 & 87.556 & 0.913    \\
		& ERASOR2~\cite{lim2023erasor2} & \textbf{99.374} & \textbf{98.497} & \textbf{0.989} \\ \midrule
		\multirow{3}{*}{8,600-8,800}
& Removert~\cite{kim2020iros}   & 81.102 & 77.173 &	0.791    \\
		& ERASOR~\cite{lim2021ral}      & 92.667 & 91.179 & 0.919    \\
		& ERASOR2~\cite{lim2023erasor2} & \textbf{99.455} & \textbf{98.193} & \textbf{0.988}    \\ \midrule
		\multirow{3}{*}{11,050-11,300}
& Removert~\cite{kim2020iros}   & 78.419 & 85.497 & 0.818    \\
		& ERASOR~\cite{lim2021ral}      & 93.146 & 97.642 & 0.953    \\
		& ERASOR2~\cite{lim2023erasor2} & \textbf{99.372} & \textbf{99.959} & \textbf{0.997}  \\ \midrule
		\bottomrule
	\end{tabular}
	}
	\label{table:static_map_building_in_synced_scans}
\end{table}


==> tables/static_map_building_in_synced_scans_0724.tex <==
\newcommand{\threemetrics}{\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} $\PRmap$ [\%] \end{tabular}}  & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}} $\RRmap$ [\%] \end{tabular}} & $\text{F}_{1}$ score}

\begin{table}[t!]
	\centering
	\captionsetup{font=footnotesize}
	\caption{Comparison of static map building approaches for the most crowded frame sequences in our dataset~($\PRmap$: Preservation Rate, $\RRmap$: Rejection Rate).}
%	\setlength{\tabcolsep}{5pt}
	{\scriptsize
	\begin{tabular}{clccc}
		\toprule \midrule
		Frame range & Method & \threemetrics \\ \midrule
		\multirow{3}{*}{2,250-2,500}
		% \multirow{3}{*}{\begin{tabular}{@{}c@{}}2,250- \\ 2,500 \end{tabular}}
		& Removert~\cite{kim2020iros}   & 85.072 & 47.170 & 0.607    \\
		& ERASOR~\cite{lim2021ral}      & 95.325 & 82.490 & 0.884    \\
		& ERASOR2~\cite{lim2023erasor2} & \textbf{99.522} & \textbf{95.339} & \textbf{0.974} \\ \midrule
		\multirow{3}{*}{8,600-8,800}
& Removert~\cite{kim2020iros}   & 80.581 & 71.965 &	0.760    \\
		& ERASOR~\cite{lim2021ral}      & 91.610 & 84.290 & 0.878    \\
		& ERASOR2~\cite{lim2023erasor2} & \textbf{99.530} & \textbf{93.740} & \textbf{0.965}    \\ \midrule
		\multirow{3}{*}{11,070-11,300}
& Removert~\cite{kim2020iros}   & 82.852 & 81.301 & 0.821    \\
		& ERASOR~\cite{lim2021ral}      & 93.969 & 89.955 & 0.919    \\
		& ERASOR2~\cite{lim2023erasor2} & \textbf{99.676} & \textbf{97.175} & \textbf{0.984}  \\ \midrule
		\bottomrule
	\end{tabular}
	}
	\label{table:static_map_building_in_synced_scans}
\end{table}


==> tables/summary_table_v1.tex <==
\begin{table}[t!]
    \captionsetup{font=footnotesize}
    \centering
    \caption{Comparison between existing 3D point cloud datasets and our proposed dataset. The tem \textit{Hetero} indicates whether a dataset includes both mechanically spinning omnidirectional and solid-state LiDAR sensors or not. We consider 2D and 3D omnidirectional LiDAR sensors as being homogeneous. The symbol - denotes that the labeled frames are not available.}
    \setlength{\tabcolsep}{3pt}
    {\scriptsize
        \begin{tabular}{l|l|cccccc}
            \toprule \midrule
            & Dataset & Year & \begin{tabular}{@{}c@{}}Multiple \\ LiDARs\end{tabular} & Hetero & \begin{tabular}{@{}c@{}}Point-wise\\ MOS \\ labels\end{tabular} & \begin{tabular}{@{}c@{}}\# of MOS- \\ labeled frames\end{tabular} \\ \midrule
            \parbox[t]{2mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{Odometry \& PR}}} &
            KITTI~\cite{geiger2012cvpr} & 2012 & \xmark  & \xmark & \xmark &  - \\
            & NCLT~\cite{carlevaris2016nclt} & 2016 & \xmark   & \xmark & \xmark &  - \\
            & Oxford Robotcar~\cite{maddern2017oxford} & 2017 & \cmark   & \xmark & \xmark &  - \\
            & Complex Urban~\cite{jeong2019complex} & 2019 & \cmark   & \xmark & \xmark &  - \\
            & MulRan~\cite{kim2020mulran} & 2020 & \xmark   & \xmark & \xmark &  - \\
            & LIBRE~\cite{carballo2020libre} & 2020 & \cmark  & \xmark & \xmark &  - \\
            & TIERS~\cite{qingqing2022tiers} &2022 & \cmark   & \cmark & \xmark & - \\
            & HeliPR~\cite{jung2023helipr} & 2023 & \cmark & \cmark    & \xmark & - \\ \midrule
            \parbox[t]{2mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{Perception}}} &
            KITTI~\cite{geiger2012cvpr} & 2012 & \xmark  & \xmark & \xmark &  - \\
            & SemanticKITTI~\cite{behley2019iccv} & 2019 & \xmark & \xmark & \cmark & 44K \\
            & nuScenes~\cite{caesar2020cvpr} & 2020 & \xmark  & \xmark & \cmark  & 40K \\
            & SemanticPOSS~\cite{pan2020semanticposs} & 2020 & \xmark & \xmark & \cmark & 3K \\
            & WOMD~\cite{ettinger2021womd} & 2021 & \cmark & \cmark & \xmark  & - \\
            & PandaSet~\cite{xiao2021pandaset} & 2021 & \cmark  & \cmark & \xmark & - \\
            & WOMD-LiDAR~\cite{chen2023womd} & 2023 & \cmark & \cmark & \xmark  & - \\
            & Proposed & 2024 & \cmark & \cmark & \cmark  & \textbf{50K} \\
            \midrule\bottomrule
        \end{tabular}
    }
    \label{table:summary}
\end{table}


==> tables/summary_table_wo_frames.tex <==
\definecolor{table1cellcolor}{rgb}{1.0,1.0,0.6}

\begin{table}[t!]
    \captionsetup{font=footnotesize}
    \centering
    \caption{Comparison between existing 3D point cloud datasets and our proposed dataset. The term \textit{Hetero} indicates whether a dataset comprises both mechanically spinning omnidirectional and solid-state LiDAR sensors. We consider 2D and 3D omnidirectional LiDAR sensors to be homogeneous to each other.
    The symbol \trimark$\,$ indicates that the dataset provides point-wise labels; however, it incorrectly labels parked vehicles as moving objects by na\"{i}vely considering all pedestrians and vehicles as in motion.}
%    \setlength{\tabcolsep}{4pt}
    {\scriptsize
        \begin{tabular}{l|l|ccccc}
            \toprule \midrule
            & Dataset & Year & \begin{tabular}{@{}c@{}}Multiple \\ LiDARs\end{tabular} & Hetero & \begin{tabular}{@{}c@{}}Point-wise\\ MOS labels\end{tabular} \\ \midrule
            \parbox[t]{5mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{ \begin{tabular}{@{}c@{}}Odometry \& \\ place recognition \end{tabular}}}} &
            KITTI~\cite{geiger2012cvpr} & 2012 & \xmark  & \xmark & \xmark  \\
            & NCLT~\cite{carlevaris2016nclt} & 2016 & \xmark   & \xmark & \xmark  \\
            & Oxford Robotcar~\cite{maddern2017oxford} & 2017 & \cmark   & \xmark & \xmark  \\
            & Complex Urban~\cite{jeong2019complex} & 2019 & \cmark   & \xmark & \xmark  \\
            & MulRan~\cite{kim2020mulran} & 2020 & \xmark   & \xmark & \xmark \\
            & LIBRE~\cite{carballo2020libre} & 2020 & \cmark  & \xmark & \xmark \\
            & TIERS~\cite{qingqing2022tiers} &2022 & \cmark   & \cmark & \xmark \\
            & HeLiPR~\cite{jung2023helipr} & 2023 & \cmark & \cmark    & \xmark \\ \midrule
            \parbox[t]{0mm}{\multirow{8}{*}{\rotatebox[origin=c]{90}{Perception}}} &
            KITTI~\cite{geiger2012cvpr} & 2012 & \xmark  & \xmark & \xmark  \\
            & SemanticKITTI~\cite{behley2019iccv} & 2019 & \xmark & \xmark & \cmark  \\
            & SemanticPOSS~\cite{pan2020semanticposs} & 2020 & \xmark & \xmark & \trimark  \\
            & nuScenes~\cite{caesar2020cvpr} & 2020 & \xmark  & \xmark & \xmark   \\
            & WOMD~\cite{ettinger2021womd} & 2021 & \cmark & \cmark & \xmark   \\
            & PandaSet~\cite{xiao2021pandaset} & 2021 & \cmark  & \cmark & \xmark  \\
            & WOMD-LiDAR~\cite{chen2023womd} & 2023 & \cmark & \cmark & \xmark \\
            & \cellcolor{table1cellcolor}HeLiMOS (Ours) & \cellcolor{table1cellcolor}2024 & \cellcolor{table1cellcolor}\cmark & \cellcolor{table1cellcolor}\cmark & \cellcolor{table1cellcolor}\cmark \\
            \midrule \bottomrule
        \end{tabular}
    }
    \label{table:summary}
\end{table}

